BaZi-Based Character Simulation Benchmark: Evaluating AI on Temporal and Persona Reasoning

Human-like virtual characters are crucial for games, storytelling, and virtual reality, yet current methods rely heavily on annotated data or handcrafted persona prompts, making it difficult to scale up and generate realistic, contextually coherent personas. We create the first QA dataset for BaZi-based persona reasoning, where real human experiences categorized into wealth, health, kinship, career, and relationships are represented as life-event questions and answers. Furthermore, we propose the first BaZi-LLM system that integrates symbolic reasoning with large language models to generate temporally dynamic and fine-grained virtual personas. Compared with mainstream LLMs such as DeepSeek-v3 and GPT-5-mini, our method achieves a 30.3%-62.6% accuracy improvement. In addition, when incorrect BaZi information is used, our model's accuracy drops by 20%-45%, showing the potential of culturally grounded symbolic-LLM integration for realistic character simulation.

==> latex/related_work_for_control_experiments.tex <==

\subsection{Related Work: Birth Timing Effects on Life Outcomes}

A growing body of empirical literature explores how birth timing—ranging from cohort-level shocks to season of birth and relative school-entry age—affects life outcomes such as education, health, and socio-economic status. \textbf{Season-of-birth effects} are well-evidenced: Crawford et al. (2014) show that differences in age at test time, rather than age at school entry, explain most academic disparities between children born early versus late in the academic year; by age seven, August-born students score lower by about 5\% of a standard deviation \cite{crawford2014drivers}. Complementing this, UK Biobank data reveal that autumn-born individuals are significantly more likely to continue full-time education after age 16, especially notable in those born in September (OR ≈ 1.43) compared to August \cite{field2015season}.

Beyond education, large-scale health record analyses uncover robust links between birth month and disease risk. The phenome-wide association SeaWAS study—covering 1.7 million New York City patients—found that those born in May had the lowest overall disease risk, while October-born individuals exhibited the highest, across 55 conditions including asthma and atrial fibrillation \cite{boland2015phenome}. This was later replicated in a cohort of over 1.1 million Mount Sinai patients, confirming the consistency of seasonal birth risks for cardiovascular conditions \cite{li2016replication}.

Some studies also investigate \textbf{prenatal timing's physiological mechanisms}: for instance, conception in colder months is associated with higher brown adipose tissue activity and lower BMI in later life \cite{seasonalreview2020}. A broader review further links season of birth to varying risks of obesity, birth weight, and body dimensions, providing biological plausibility for these associations \cite{seasonalreview2020}. Moreover, immune-mediated diseases (e.g., multiple sclerosis, rheumatoid arthritis) display modest seasonal birth patterns potentially tied to in utero vitamin D exposure \cite{vitamind2012}.

In stark contrast, \textbf{astrological systems}—zodiac signs, Chinese zodiac, natal charts, or BaZi—lack credible empirical support. Classical tests, including Carlson’s double-blind study, and large-scale meta-analyses consistently show astrologers perform no better than chance in predicting personality or life outcomes. These findings emphasize the absence of predictive validity for traditional astrological frameworks in comparison with empirically robust temporal variables.

Taken together, the evidence highlights that well-documented temporal markers—such as birth month/season, relative age effects, and prenatal environmental conditions—demonstrably influence educational and health trajectories. Conversely, astrological indicators provide no predictive advantage. This motivates our study: we compare a baseline model using conventional temporal variables (birth year, zodiac, birth month/quarter, and birth hour) to a full model incorporating BaZi and natal chart-derived features, assessing whether traditional divinatory constructs capture any incremental predictive signal beyond established temporal influences.


